The Super-Puff WASP-193b is On A Well-Aligned Orbit

The "super-puffs" are a population of planets that have masses comparable to that of Neptune but radii similar to Jupiter, leading to extremely low bulk densities ($\rho_p \lesssim 0.2\,\mathrm{g}\,\mathrm{cm}^{-3}$) that are not easily explained by standard core accretion models. Interestingly, several of these super-puffs are found in orbits significantly misaligned with their host stars' spin axes, indicating past dynamical excitation that may be connected to their low densities. Here, we present new Magellan/PFS RV measurements of WASP-193, a late F star hosting one of the least dense transiting planets known to date ($M_p = 0.112^{+0.029}_{-0.034}\,M_J$, $R_p = 1.319^{+0.056}_{-0.048}\,R_J$, $\rho_p = 0.060\pm0.019\,\mathrm{g}\,\mathrm{cm}^{-3}$). We refine the bulk properties of WASP-193 b and use interior structure models to determine that the planet can be explained if it consists of roughly equal amounts of metals and H/He, with a metal fraction of $Z = 0.42$. The planet is likely substantially re-inflated due to its host star's evolution, and expected to be actively undergoing mass loss. We also measure the projected stellar obliquity using the Rossiter-McLaughlin effect, finding that WASP-193 b is on an orbit well-aligned with the stellar equator, with $\lambda = 17^{+17}_{-16}$ degrees. WASP-193 b is the first Jupiter-sized super-puff on a relatively well-aligned orbit, suggesting a diversity of formation pathways for this population of planets.

==> rv_table.tex <==
% bjdtdb, rv, rverr, exptime
2460300.84220 & -5.39 & 6.99 & 600 \\
2460333.83057 & 7.53 & 5.20 & 600 \\
2460337.85463 & -18.99 & 5.62 & 600 \\
2460338.82387 & -0.29 & 5.78 & 600 \\
2460341.81969 & 2.59 & 5.22 & 600 \\
2460367.53478 & -14.13 & 6.87 & 900 \\
2460367.54523 & 6.74 & 5.38 & 900 \\
2460367.55428 & 0.00 & 6.91 & 600 \\
2460367.56132 & 16.18 & 6.23 & 600 \\
2460367.56872 & 26.64 & 5.84 & 600 \\
2460367.57589 & 44.94 & 5.60 & 600 \\
2460367.58310 & 63.47 & 5.49 & 600 \\
2460367.59022 & 40.57 & 6.08 & 600 \\
2460367.59771 & 39.85 & 5.75 & 600 \\
2460367.60479 & 41.58 & 5.74 & 600 \\
2460367.61194 & 38.86 & 5.83 & 600 \\
2460367.61943 & 38.50 & 5.32 & 600 \\
2460367.62651 & 24.38 & 5.41 & 600 \\
2460367.63384 & 30.25 & 4.92 & 600 \\
2460367.64074 & 12.64 & 5.59 & 600 \\
2460367.64831 & -2.33 & 5.62 & 600 \\
2460367.65552 & -1.44 & 5.27 & 600 \\
2460367.66265 & -14.56 & 5.01 & 600 \\
2460367.66999 & -16.64 & 5.22 & 600 \\
2460367.67716 & -33.48 & 5.01 & 600 \\
2460367.68434 & -37.30 & 5.22 & 600 \\
2460367.69172 & -33.06 & 6.41 & 600 \\
2460367.69892 & -57.64 & 5.74 & 600 \\
2460367.70623 & -51.46 & 5.34 & 600 \\
2460367.71333 & -52.64 & 5.81 & 600 \\
2460367.72069 & -39.13 & 5.20 & 600 \\
2460367.72845 & -20.66 & 5.05 & 600 \\
2460367.73604 & 5.90 & 5.84 & 600 \\
2460367.74327 & -18.13 & 5.58 & 600 \\
2460367.75039 & -1.33 & 4.63 & 600 \\
2460367.75760 & -5.55 & 4.82 & 600 \\
2460367.76484 & 11.24 & 4.94 & 600 \\
2460367.77215 & -0.10 & 5.54 & 600 \\
2460367.77917 & 11.14 & 5.36 & 600 \\
2460367.78654 & 1.26 & 5.75 & 600 \\
2460367.79381 & -14.06 & 5.84 & 600 \\
2460371.72535 & 7.35 & 5.66 & 600 \\
2460372.71509 & 7.44 & 5.74 & 600 \\
2460374.71837 & -13.37 & 5.66 & 600 \\
2460457.51177 & -41.93 & 7.97 & 600 \\
2460460.50643 & 6.31 & 5.36 & 600 \\
2460461.51074 & 1.37 & 6.04 & 600 \\
2460462.51176 & 29.32 & 7.54 & 600 \\
2460463.49162 & -10.45 & 5.37 & 600 \\

